Combinatorial Multivariant Multi-Armed Bandits with Applications to Episodic Reinforcement Learning and Beyond

We introduce a novel framework of combinatorial multi-armed bandits (CMAB) with multivariant and probabilistically triggering arms (CMAB-MT), where the outcome of each arm is a $d$-dimensional multivariant random variable and the feedback follows a general arm triggering process. Compared with existing CMAB works, CMAB-MT not only enhances the modeling power but also allows improved results by leveraging distinct statistical properties for multivariant random variables. For CMAB-MT, we propose a general 1-norm multivariant and triggering probability-modulated smoothness condition, and an optimistic CUCB-MT algorithm built upon this condition. Our framework can include many important problems as applications, such as episodic reinforcement learning (RL) and probabilistic maximum coverage for goods distribution, all of which meet the above smoothness condition and achieve matching or improved regret bounds compared to existing works. Through our new framework, we build the first connection between the episodic RL and CMAB literature, by offering a new angle to solve the episodic RL through the lens of CMAB, which may encourage more interactions between these two important directions.

==> content/x_icml_rebuttal.tex <==
\section{Rebuttal}
\subsection{Rebuttal to bJUc, score 7}
We thank the reviewer for their positive feedback about our work's contribution to both CMAB-T and episodic RL domains.

\textbf{Q1. About multivariant distributions beyond the multinoulli distribution.}
Our work can also handle the $\sigma$-norm-subGaussian multivariant random variables (denoted as nSG($\sigma$)), defined in the Definition 3 of [1] as follows:

\begin{definition}
    A random vector $\boldsymbol{X}\in \R^d$ is a norm-subGaussian (or nSG($\sigma$)), if there exists $\sigma$ so that:
    \begin{align}
        \Pr[\norm{\boldsymbol{X}-\mathbb{E}[\boldsymbol{X}]}\ge t]\le 2 e^{-\frac{t^2}{2\sigma^2}}.
    \end{align}
\end{definition}

Notably, any bounded multivariant random variables $\boldsymbol{X}\in \mathbb{R}^d$ with $||\boldsymbol{X}||_2\le \sigma$ are nSG($\sigma$). Leveraging corollary 7 in [1], $||\hat{\boldsymbol{X}}_n-\mathbb[\boldsymbol{X}]||_2 \le c\sqrt{\sigma\log \frac{2d}{\delta}/n}$ with probability at least $1-\delta$, where $\hat{\boldsymbol{X}}_n$ denotes the empirical mean after $n$ rounds of observation and $c$ represents a constant. The right-hand side yields a $O(\sqrt{d})$ factor improvement compared to treating $\boldsymbol{X}$ as $d$ separate $\sigma$-subGaussian random variables. This means our framework can handle applications with arms being any bounded multivariant random variables beyond multinoulli, achieving $O(\sqrt{d})$ improvements.

[1]. Jin, Chi, Praneeth Netrapalli, Rong Ge, Sham M. Kakade, and Michael I. Jordan. "A short note on concentration inequalities for random vectors with subgaussian norm." arXiv preprint arXiv:1902.03736 (2019).

\textbf{Q2. Regarding the presentation of Theorem 1.}

We thank the reviewer for this valuable suggestion. For conditions (1), (3) in Theorem 1, as suggested by the reviewer, we will revise our presentation in the final version to emphasize that these conditions should hold with high probability rather than definitely. 
For Theorem 1, our main focus is to offer a general solution characterized by parameters $F,G,I,J$, capable of adapting to a wide range of applications. For Remark 5, we give some initial results by realizing $F,G,I,J$ for some special cases (e.g., CMAB-T with Bernoulli random variables) for the audience to understand our results. We leave the detailed realizations of $F,G,I,J$ for tight regret bounds for subsequent applications. As suggested by the reviewer, we can write out the bounds for special cases in Remark 5 as separate corollaries in the final version. Following the reviewer's suggestion, we plan to revise the presentation of Theorem 1 as follows:

Fix the underlying distribution $D \in \mathcal{D}$ and its mean vector $\bmu\in [0,1]^{m\times d}$ with optimal action $\pi^*$.
Recall that for any round $t$, $\hat{\boldsymbol{\mu}}_{t-1,i}$ is the empirical mean, $\tilde{\mathcal{C}}_t$ is the confidence region function defined in Eq. (1) with problem-specific parameters $F_{t,i}$ and $I_{t,i}$, $\tilde{\mathcal{O}}$ is the joint oracle, and $(\pi_t,\tilde{\boldsymbol{\mu}}_{t})=\tilde{\mathcal{O}}(\mathcal{C}_t)$ are the pair of optimistic policy and parameter in line 4 of Algorithm 1. Define the concentration event 
\begin{equation*}
	\mathcal{E}_1 = \left\{ |(\boldsymbol{\mu}_i-\hat{\boldsymbol{\mu}}_{t-1,i})^{\top}\boldsymbol{w}^{\boldsymbol{\mu},\pi^*}_i| \le 
	 F_{t,i}\sqrt{\frac{1}{N_{t-1,i}}}+I_{t,i}\frac{1}{N_{t-1,i}}, \text{ for all } i\in[m], t\in[T] \right\}.
\end{equation*}
Let $G_{t,i}, J_{t,i}$ be another two problem-specific parameters for $i\in[m],t\in[T]$, and define the second concentration event 
$$\mathcal{E}_2 = \left\{|(\boldsymbol{\mu}_i-\hat{\boldsymbol{\mu}}_{t-1,i})^{\top}(\boldsymbol{w}^{\tilde{\boldsymbol{\mu}},\pi_t}_i-\boldsymbol{w}^{\boldsymbol{\mu},\pi^*}_i)|\le G_{t,i}\sqrt{\frac{1}{N_{t-1,i}}}+J_{t,i}\frac{1}{N_{t-1,i}}, \text{ for all } i\in[m], t\in[T] \right\}.$$ 
Let $\bar{F},\bar{G}, \bar{I},\bar{J}$ be upper bounds for problem specific parameters so that $\sum_{i\in[m]}q_i^{\bmu,\pi_t}F_{t,i}^2\le \bar{F}$, $\sum_{i\in[m]}q_i^{\bmu,\pi_t}G_{t,i}^2\le \bar{G}$, $I_{t,i}\le \bar{I}$, $J_{t,i}\le \bar{J}$, then we have the following theorem.

\begin{theorem}\label{thm:reg_CMAB-MT2}
    For a CMAB-MT problem instance $([m], d, \Pi, \cD, D_{\text{trig}},R)$ that satisfies 1-norm MTPM smoothness condition (Condition \ref{cond:general_smooth}) with weight vectors $\bw_i^{\tilde{\bmu},\pi}\in [0,\bar{w}]^d$ for $\tilde{\bmu}\in[0,1]^{m\times d},\pi\in\Pi,i\in[m]$,
    if the oracle $\tilde{\cO}$ is an $(\alpha,\beta)$-approximation oracle, and concentration events $\mathcal{E}_1,\mathcal{E}_2$ hold with probability at least $1-\frac{1}{T}$, then CUCB-MT (Algorithm 1) 
    achieves an $(\alpha,\beta)$-approximate gap-dependent regret bounded by
    \begin{align}
        O\left(\sum_{i \in [m]} \frac{(\bar{F}+\bar{G})}{\Delta_{i}^{\min} } + (\bar{I}+\bar{J})  \log\left (\frac{(\bar{I}+\bar{J})K}{\Delta_{i}^{\min}}\right)\right),
    \end{align}
and the gap-independent regret bounded by
\begin{align}
O\left(\sqrt{m(\bar{F}+\bar{G})T}+m(\bar{I}+\bar{J})\log (KT)\right).
\end{align}
\end{theorem}

$\mathcal{E}_1$ represents the previous condition (1) such that $\boldsymbol{\mu}\in \mathcal{C}_t(\pi^*)$ for all $t\in[T]$ and $\mathcal{E}_2$ represents the previous condition (3), which are required to hold with probability at least $1-1/T$. 
As mentioned in Remark 5, both $\mathcal{E}_1$ and $\mathcal{E}_2$ are concentrations of $\hat{\boldsymbol{\mu}}_{t-1,i}$ around $\boldsymbol{\mu}$, but $\mathcal{E}_2$ may concentrates faster since $(\boldsymbol{w}^{\tilde{\boldsymbol{\mu}},\pi_t}_i-\boldsymbol{w}^{\boldsymbol{\mu},\pi^*}_i)$ could be quite small when $t$ increases, yielding tighter regret bounds.

We can also give the following two corollaries for some special cases as previously stated in Remark 5.
\begin{corollary}
    For any CMAB-MT instance that satisfies 1-norm MTPM smoothness condition with weight vectors $\bw_i^{\tilde{\bmu},\pi}\in [0,\bar{w}]^d$ for $\tilde{\bmu}\in[0,1]^{m\times d},\pi\in\Pi,i\in[m]$, when base arms follow the $d$-dimensional multinoulli distribution, we have $\bar{F}=\bar{G}=O(\bar{w}^2Kd\log T), {I}=\bar{J}=0$ and the $(\alpha,\beta)$-regret given by Algorithm 1 is bounded by $O\left(\bar{w}\sqrt{dmKT\log T}\right)$.
\end{corollary}

\begin{corollary}
For any CMAB-T instance that satisfies 1-norm TPM smoothness condition with coefficient $B_1$, when base arms follow Bernoulli distribution, we have $\bar{F}=O(\bar{B}_1^2K\log T), \bar{G}=\bar{I}=\bar{J}=0$ and the $(\alpha,\beta)$-regret given by Algorithm 1 is bounded by $O\left(B_1\sqrt{mKT\log T}\right)$.
\end{corollary}


\textbf{Q3. About the PMC-GD application.}
PMC-GD is a variant of the probabilistic maximum coverage problem (PMC), where each source node can cover exactly one target node following the multinoulli distribution. This can be motivated by the goods distribution application, where the source node wants to randomly distribute one good (e.g., coupon, product, food) to exactly one of the target users. We can extend this model to randomly distribute $c$ goods to any set of $c$ users, i.e., the multivariant random variable $X\in \mathbb{R}^d$ has $c$ ones and $(d-c)$ zeros in $X$, where $c$ is some constant. This setting could be more realistic than the current setting in the submission. 
As mentioned in Q1, such variables $\boldsymbol{X}$'s are norm-subGaussian random variables $\boldsymbol{X}\in nSG(c)$, which results in similar improvements as in PMC-GD.

\textbf{Q4. About the constant factors.}
Due to the space limit, all constant factors are presented in the appendix. For example, Eq. (61) gives the regret bound for Theorem 1, i.e., $\text{Reg}(T)\le\sum_{i \in [m]} \frac{144(\bar{F}+\bar{G})}{\Delta_{i}^{\min} } (3+ \log K) + \sum_{i\in [m]} 12(\bar{I}+\bar{J})  \left(1+\log\left (\frac{12(\bar{I}+\bar{J})K}{\Delta_{i}^{\min}}\right)\right) + 3m\bar{w}d$. We will state the exact constant factors in our main content in the final version.

\textbf{Q5. About the action-dependent confidence region $\mathcal{C}(\pi)$.}
The dependency of $\pi$ for the confidence region defined in Eq. (1) comes from the weight vector $\boldsymbol{w}^{\tilde{\boldsymbol{\mu}},\pi}_i$. This formulation aligns closely with the 1-norm MTPM condition (Condition 1). So similar to Condition 1, if we fix the weight vector to $\bar{\boldsymbol{w}}$ that is independent of $\pi$, then the confidence region or Condition 1 reduces to standard region/condition, potentially quite loose. In fact, the similar action-dependent confidence region is also used in efficient sampling for combinatorial bandits (ESCB) algorithm (Combes et al., 2015), where the confidence is tailored to each super-arm $\pi$, resulting in 
 a tighter regret bound compared to the action-independent confidence region used in CUCB algorithms (Chen et al., 2013b, Wang and Chen, 2018).

As mentioned by the reviewer, for most applications, we can replace $\mathcal{C}(\pi)$ with $\mathcal{C}$, as what we do for episodic RL in section 4.3 and PMC-GD application in section 5. In section 4.4, however, an action-dependent confidence region is essential for achieving the minimax optimal regret in episodic RL, as demonstrated in Eq. (7), where the weight $V_{h+1}^{\tilde{p},\pi}$ is associated with action $\pi$. 

 

\textbf{Q6. About the coefficient $K'$.}
We thank the reviewer for pointing out this, it should be $K'=SH$ since the action $a_h$ is chosen deterministically at step $h$. Only when the action is not deterministic, $K'=SAH$.

\textbf{Q7. About the simplification of the proof.}
We thank the reviewer for pointing out the possible improvement in the proof. When $F_{t,i}, G_{t,i}$ are upper bounded by constants $C$ for all $i\in [m], t\in[T]$, we can follow exactly the reviewer's method to simplify the proof and improve the constant factors. However, when $\sum_{i\in [m]}q_i^{\mu,\pi_t}F_{t,i}^2\le \bar{F} \ll KC^2$, using one step of Cauchy-Swartz in step (e) can yield tighter regret bound. We use this trick, together with the variance-aware analysis, to obtain the minimax-optimal regret in section 4.4, where $F_{t,i}^2$ is related to the variance of the arm. We will put this discussion in the final version.


\subsection{Rebuttal to XMoy, score: 7}
We thank the reviewer for their positive feedback about our work's novelty and its potential for a broader impact.

\textbf{Q1. About the strictness of the condition 1.}
Condition 1 (1-norm MTPM smoothness) is a general and flexible condition that can cover a wide range of applications, facilitated through the adaptable weight vectors. As highlighted in Remark 3 in line 173, with $d=1$ and $w_i^{\tilde{\mu},\pi}$ being a 1-dimensional weight vector $B_1$, our condition 1 reduces to the classical 1-norm TPM condition with coefficient $B_1$ in CMAB-T setting, which covers a variety of practical applications,  including cascading bandits (Kveton et al., 2015a, 2015b), online influence maximization (Wen et al., 2017, Wang and Chen, 2017), etc. When $d>1$, Condition 1 covers the episodic RL and PMC-GD applications investigated in our study. Moreover, We believe our condition has great potential to cover more practical applications, where one can select appropriate weight vectors $w_i^{\tilde{\mu},\pi}$, achieving tight regret bounds using our algorithm and results in Theorem 1.


\textbf{Q2. About the assumption that the reward distributions are known in the episodic RL setting}
Learning the unknown reward distributions poses no real difficulty compared with learning the unknown transition kernel, so similar to Assumption 1 in Azar et al., 2017, we assume reward distributions are known.
In fact, the unknown reward distribution $\mathcal{R}$ can be handled by treating them as an additional group of base arm of $ (s,a,h) \in \mathcal{S}\times \mathcal{A} \times [H]$ base arms with $d=1$, whose distribution is Bernoulli with unknown mean $\mu_{s,a,h}=r(s,a,h)$. Now we have $m=2SAH$ base arms and the new $SAH$ arms can be integrated into our framework by validating Condition 1 with weight $w_{s,a,h}^{\tilde{\mu},\pi}=1$ and $q_{s,a,h}^{\mu,\pi}$ being the occupancy measure of $(s,a,h)$ for each new base arm, yielding an additional $\tilde{O}(\sqrt{H^2SAT})$ regret term. The final regret bound remains the same since the additional regret term is dominated by the $\tilde{O}(\sqrt{H^3SAT})$ regret, which is caused by the unknown transition. We will add a detailed discussion in the final version.
% \siwei{Why not just add a dimension (so that the observation is with dimension $|S|+1$)?}
% In fact, the unknown reward distribution $\mathcal{R}$ can be handled by adding an additional dimension to each base arm $ (s,a,h) \in \mathcal{S}\times \mathcal{A} \times [H]$, whose distribution is Bernoulli with unknown mean $r(s,a,h)$. Now each new base arm $(s,a,h)$ corresponds to $\mu_{s,a,h}=[p(s,a,h),r(s,a,h)]\in \mathbb{R}^{S+1}$. These new $SAH$ arms with $d=S+1$ can fit into our framework by validating Condition 1 and Lemma 2 with weight vector $w_{s,a,h}^{\tilde{\mu},\pi}=[V^{\tilde{\mu},\pi}_{h+1},1]\in \mathbb{R}^{S+1}$ where weight $1$ corresponds to the unknown reward distribution, yielding an additional $\tilde{O}(\sqrt{H^2SAT})$ regret term. The final regret bound remains the same since the additional regret term is dominated by the $\tilde{O}(\sqrt{H^3SAT})$ regret, which is caused by the unknown transition. We will add a detailed discussion in the final version.

\textbf{Q3. About the comparison of the existing results.}
For the gap-dependent bound, since we use very different CMAB proof techniques in our analysis, the definition of our suboptimality gap is different from the gap in [Simchowitz and Jamieson, 2019], so it is hard to directly compare with them. Therefore, in Appendix E.5, we reformulate our gap definition to align with [Simchowitz and Jamieson, 2019], facilitating a more coherent comparison. For the gap-independent bound, all our definitions and assumptions are consistent with existing work (Jaksch et al., 2010, Azar et al., 2017, Zanette and Brunskill, 2019). To enhance the clarity, we will add a table including detailed assumptions and comparisons with existing works in our final version.

\textbf{Q4. The generalization of the current work.}
In our work, we need to know the mean reward function $r(\pi;\mu)$ to design the explicit joint oracle which yields the $(\alpha,\beta)$-approximate solution. However, if we assume that an oracle is given, we do not need to assume that the reward function is known anymore.
For other generalizations, as mentioned in the conclusion and future work section, one interesting direction is to consider linear or nonlinear function approximation for the CMAB-MT framework, which could cover broader applications and give matching or tighter results for RL problems with general function approximation.


\subsection{Rebuttal to tnew, score: 5}
We thank the reviewer for their positive feedback.

\textbf{Q1. Regarding the advantages of employing the CMAB-MT framework for episodic RL}
The main contribution of this work lies in introducing a general and unified CMAB-MT framework, which not only covers the existing applications of CMAB-T framework but also extends its applicability to new domains such as tabular episodic RL and PMC-GD, either matching or enhancing the regret bounds previously established. Specifically, for the tabular episodic RL, our framework uses a unified approach to achieve both a minimax gap-independent regret bound and a gap-dependent regret bound that is at most $O(1/q^*)$ factor larger than the existing works. This represents our first advantage. Importantly, as mentioned in the discussion of Theorem 3, using our CMAB-MT framework with sharp CMAB proof techniques yields an improvement by a factor of $O(\log^{5/2}(SAHT))$ in the leading $O(\sqrt{T})$ term for the gap-independent regret, compared to \cite{zanette2019tighter}, which is the second benefit. Regarding computational complexity, our framework is on par with seminal works in the field (Jaksch et al., 2010, Zanette and Brunskill, 2019), thereby asserting its theoretical and practical efficacy.



\textbf{Q2. The example of receiving feedback from arms other than the super arm in CMAB-MT (or CMAB-T) setting}
One example of receiving feedback from arms beyond the selected super arm is the online influence maximization (OIM) application,as explored by Wen et al. (2017) and Wang and Chen (2017). In OIM problem under the independent cascade model, consider a weighted directed graph $G(V,E,p)$, where $V$ is the set of vertices, $E$ is the set of directed edges, and each edge $(u,v)\in E$ is associated with a probability $p(u,v)\in [0,1]$. When the agent selects a set of seed nodes $S \subseteq V$, the influence propagation process is as follows: At time $0$, the seed nodes in $S$ are activated; At time $t > 1$, a node $u$ activated at time $t-1$ will have one chance to activate its inactive out-neighbor $v$ with independent probability $p(u,v)$. The influence spread of $S$ is denoted as $\sigma(S)$ and is defined as the expected number of activated nodes after the propagation process ends. The problem of influence maximization is to find seed nodes $S$ with $|S|\le k$ so that the influence spread $\sigma(S)$ is maximized. 

In this context, the super arm refers to the set of edges $E_S$ which are the out-edges of the seed nodes $S$. The agent not only can observe the edge feedback of $E_S$ (i.e., whether $u$ successfully activates $v$ for $(u,v)\in E_S$), but can also observe the feedback of edges $E_{\tilde{S}}$ that are out-edges of all activated nodes $\tilde{S}$, where $E_S\subseteq E_{\tilde{S}}$. Hence, the agent can receive feedback from a broader set of arms $E_{\tilde{S}}$, extending beyond the super arm $E_S$.


\textbf{Q3. About the assumption of the fixed initial states.}
For the ease of exposition, we assume the initial states are fixed to $s_1$.
However, our framework can handle the case where initial state $s_{t,1}$ in episode $t$ is not fixed but follows a (unknown) distribution $p_1 \in \Delta_S$.
Specifically, we can add a virtual starting state $s_0$ with only one feasible action $a_0$ that leads to $0$ reward and transits to the initial state $s_{t,1}$ following unknown distribution $p_1$. In this case, it is equivalent to learn a new episodic RL with $H+1$ steps $\{0,1,...,H\}$, where $p_1$ can be treated as a new base arm $(s_0,a_0,1)$ that can be learned by our framework. Then we can change the regret definition in Eq. (5) to be $\text{Reg}(T)=\sum_{t \in [T]}\left(V_{0}^{*}(s_0)-V_{0}^{\pi_t}(s_0)\right)$. Then we can verify that Lemma 1 (and Lemma 2) still holds with $s_1$ changed to state $s_0$ and with $q_{s,a,h}^{p,\pi}$ corresponding to the occupancy measure of $(s,a,h)$ starting from the initial state $s_{0}$. Finally, our results remain almost unchanged (except that number of base arms is now $SAH+1$ and the horizon is now $H+1$) by following the same algorithm and analysis with initial state $s_{0}$ in each episode $t$. 

% For the ease of exposition, we assume the initial states are fixed to $s_1$. However, our framework can handle any initial states $s_{t,1}$ in episode $t$, which may follow a known distribution $p_{1}$ (or even different $p_{t,1}$ for episode $t$) specified by the environment. 
% Specifically, we can change the regret definition in Eq. (5) to be $\text{Reg}(T)=\sum_{t \in [T]}\left(V_{1}^{*}(s_{t,1})-V_{1}^{\pi_t}(s_{t,1})\right)$. Then we can verify that Lemma 1 (and Lemma 2) still holds with $s_1$ changed to any state $s_{t,1}$ and with $q_{s,a,h}^{p,\pi}$ corresponding to the occupancy measure of $(s,a,h)$ starting from the initial state $s_{t,1}$. Finally, our results remain the same by following the same algorithm and analysis with initial states $s_{t,1}$ in each episode $t$. 

% Moreover, for unknown initial distribution $p_{1}$, we can add a virtual starting state $s_0$ with only one feasible action $a_0$ that leads to $0$ reward and transits to the initial state $s_{t,1}$ following unknown distribution $p_1$. In this case, it is equivalent to learn a new episodic RL with $H+1$ steps, where $p_1$ can be treated as a new base arm $(s_0,a_0,1)$ that can be learned by our framework. 


\textbf{Q4. On the limitation of the current work}
One limitation of the current work is that the current work cannot give the optimal gap-dependent regret bound for episodic RL. We conjecture that this limitation arises from our general CMAB-MT analysis, which may overlook some finer RL structures. For example, we only focus on the smoothness of the value function $V_1$ instead of all subsequent value functions $V_h$ for $h\in [H]$). This may limit our ability to identify and exploit tighter sub-optimality gaps.  In response to this limitation, we plan to conduct further research aimed at building tighter gap-dependent regret bounds for episodic RL, which may also contribute to the CMAB literature by possibly enhancing their gap-independent regret bounds.


==> content/x_linear_extension.tex <==
\clearpage
\section{Variance-Adaptive Algorithms for Linear Contextual Combinatorial Multi-Armed Bandits}
Our goal is to apply our TPVM or VM condition to the contextual combinatorial bandits, with the hope of removing $\sqrt{K}$ factor of previous results $\tilde{O}(\frac{d}{p^*}\sqrt{KT})$ \cite{li2016contextual}. For simplicity, we consider the non-triggering CMAB for now.

\subsection{Setting}
Our setting is similar to that of \cref{sec: problem setting}, the difference is that we now have a feature map $\phi:[m]\rightarrow \R^d$, an unknown parameter vector $\btheta^*\in \R^d$, and the mean reward $\mu_i = \inner{\boldsymbol{\phi(i)},\btheta^*}$ for $i \in [m]$. At each time $t$ and given history $\cH_t$, the outcome $X_{t,i}=\mu_i + \eta_{t,i}$ of arm $i$ is bounded within $[0,1]$. We assume $X_{t,i}$ is a random variable with $\E[\eta_{t,i}|\cH_t]=0$, $\E[\eta_{t,i}^2|\cH_t]\le \sigma_i^2 $, are \textbf{independent} across arm set.
To this end, we can rewrite $r(S;\bmu)=r(S;\btheta^*,\phi)$ and $S^*=\arg\max_{S \in \cS}r(S;\btheta^*,\phi)$.

Note that we can extend to time-variant contexts, i.e., $\phi_t$ and define $S_t^*=\arg\max_{S \in \cS} r(S;\btheta^*, \phi_t)$. 
The $(\alpha, \beta)$-approximate regret is defined as
\begin{align}
     Reg(T;\alpha, \beta)= \sum_{t=1}^T \alpha\beta \cdot r(S_t^*;\btheta^*, \phi_t)-\E\left[\sum_{t=1}^Tr(S_t;\btheta^*,\phi_t)\right].
\end{align}

Let $\Phi_t=[\phi_{t,1}, ..., \phi_{t,m}]\in \R^{d \times m}$, the reward is $\inner{\Phi^{\top}\theta, S_t}=\inner{\theta, \Phi S_t}=\theta^{\top} \Phi S_t$. $\tilde{\btheta}_{t}(i)=\arg\max_{i \in [m]}{\hat{\btheta}_t+\frac{(G_{t})^{-1}\phi_{t,i}}{\norm{(G_{t})^{-1/2}\phi_{t,i}}_2}}$.

\subsection{Algorithm}
\begin{algorithm}[h]
	\caption{BC$^2$UCB-T: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Known Variance Upper Bound $\bar{\sigma}_i^2$}\label{alg:BC^2UCB-T_known}
			\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, known variance upper bound $\bar{\sigma}_i$, computation oracle ORACLE.
	   % \OUTPUT Budget allocation $\bk$.
	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
	   \For{$t=1, ...,T$ }
	   \State $\hat{\btheta}_{t}=\bG_{t-1}^{-1}\bb_{t-1}$. \Comment{Compute the empirical estimator.}
	   %\State Construct the confidence set, one for decision, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$.
	   \For{$i \in [m]$}
	    \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + \sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}$.
	    \Comment{UCB value for base arm $i$.}
	    \State $\bar{\mu}_{t,i} =\min\{\bar{\mu}_{t,i},1\} $
	    \EndFor
	   %\State $G_t=\lambda \boldsymbol{I} + \sum_{\tau < t}\bphi(i)\bphi(i)^{\top}$.
	   %$\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1, i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.
	   %\State Set UCB value $\bar{\mu}_{t,i}=\min \{\hat{\mu}_{t-1, i}+\rho_{t, i},1\}$.
	   %\State $S_t=\text{ORACLE}(C_t^{\theta}, \phi_t)$.  \qquad\qquad\qquad\qquad\qquad//$S_t=\arg\max_{S \in \cS, \bnu \in C_t^{\theta}} r(S;\bnu, \phi_t)$.
	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. \Comment{Computational oracle using UCBs.}
	    \For{$ i \in \tau_t$ } \Comment{Update statistics using the triggered arms' observation.}
	   %\State $v_{t,i}=\max_{\bnu \in C^{v}_{t}}\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})$.
	   \State $\bG_t=\bG_{t-1}+ (\bar{\sigma}_i^2)^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
	   \State $\bb_t=\bb_{t-1}+ (\bar{\sigma}_i^2)^{-1}\bphi_{t}(i) X_{t,i}$.
	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
	   % \label{line:trigger_upd}
	   \EndFor
	    	   \EndFor
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}
Inspired by \cite{lattimore2015linear,zhou2021nearly,vial2022minimax}, we adopt the weighted ridge-regression to learn the unknown parameter $\theta^*$. 
Intuitively, if we know an upper bound of $\sigma_i$,  which we denote as $\bar{\sigma}_i$, and we only select one arm each round (i.e., $K=1$), then $\hat{\btheta}_t$ is the closed form solution of the following \textit{weighted ridge regression} problem:
\begin{align}
    \hat{\btheta}_t = \arg\min_{\btheta \in \R^d} \sum_{\tau=1}^{t}\sum_{i \in S_{\tau}}(\inner{\btheta, \bphi_\tau(i)}-X_{\tau,i})/\bar{\sigma}_i^2 + \lambda \norm{\btheta}_2^2.
\end{align}
The term ``weighted" corresponds the variance upper bound $\bar{\sigma}$. The above estimator is known as the best linear unbiased estimator (BLUE)~\cite{henderson1975best}. Concretely, $\hat{\btheta}_t$ is the lowest variance estimator of $\btheta$ among all unbiased linear estimators.

For our problem, we have three key ingredients: (1) We use $v_{t,i}$ is an estimation of $\bar{\sigma}_i$ at round $t$ instead of assuming a known upper bound $\bar{\sigma}_i$; (2) At each round, we select a combinatorial action which consists of multiple arms, i.e., $K > 1$. (3) We incorporate VM condition (\cref{cond:VM}) to remove the factor of $\sqrt{K}$.

\subsection{Analysis}
\subsubsection{Known Variance Upper Bound}
Suppose we know an upper bound of $\sigma_i$, i.e., $\bar{\sigma}_i^2=C_1^2\sigma_i^2$ for some $C_1^2 \ge 1$.
\begin{align}
    Reg(T) &= \sum_{t=1}^T \alpha r(S_t^*; \btheta^*, \phi_t) - r(S_t; \btheta^*, \phi_t) \\
    &\le \sum_{t=1}^T  r(S_t^*; \tilde{\btheta}_t, \phi_t)- r(S_t; \btheta^*, \phi_t) 	& \mbox{$(\tilde{\btheta}_t, S_t)=\arg\max_{S \in \cS, \btheta \in C_t^{\theta}}r(S;\btheta,\phi_t)$} \label{apdx_eq: linear_mono}\\
    &\le\sum_{t=1}^T B_v\sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}{\sigma_i^2}} 	& \mbox{\cref{cond:VM} with $\zeta_i = \inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}$}\label{apdx_eq: linear_use_cond_VM}\\
    &=\sum_{t=1}^T B_vC_1\sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}{\bar{\sigma}_i^2}} 	& \mbox{$\bar{\sigma}_i^2=C_1^2\sigma_i^2$}\\
   &\le\sum_{t=1}^T B_vC_1\sqrt{\sum_{i \in S_t}\frac{\norm{\tilde{\btheta}_t-\btheta^{*}}_{\bG_t}^2\norm{ \bphi_t(i)}_{\bG_t^{-1}}^2}{\bar{\sigma}_i^2}} 	& \mbox{Cauchy–Schwarz Inequality}\\
   &\le\sum_{t=1}^T B_vC_1\sqrt{\beta\sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}} 	& \mbox{the definition of $C_t^{\theta}$}\\
   & \le B_vC_1\sqrt{\beta}\sqrt{T\sum_{t=1}^T \sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}} 	& \mbox{Cauchy–Schwarz Inequality over $t$}\\
   & \le B_vC_1d\sqrt{T}\log T,
 \end{align}
 where the last inequality uses $\beta \le \tilde{O}(d\log (KT))$ (Theorem 3~\cite{zhou2021nearly}), and the potential lemma $\sum_{t=1}^T \sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}\le \tilde{O}(d\log (KT))$ (Eq. (44)~\cite{zhou2021nearly}).
 
 Intuitively, the source of improvement comes from the saving of one use of Cauchy-Schwarz from the 1-norm TPM condition from \cref{apdx_eq: linear_use_cond_VM}: 
 \begin{align}
      Reg(T)&\le\sum_{t=1}^T B_1 \sum_{i \in S_t}\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}\\
     &\le \sum_{t=1}^T B_1 \sqrt{ K\sum_{i \in S_t}\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}
 \end{align}

\subsection{Unknown Variance}
% \begin{algorithm}[h]
% 	\caption{BC$^2$UCB: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Unknown Variance but with Monotonicity Assumption}\label{alg:BC^2UCB-T}
% 			\resizebox{.99\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
% 	\begin{algorithmic}[1]
% 	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, computation oracle ORACLE.
% 	   % \OUTPUT Budget allocation $\bk$.
% 	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0},$ optimistic variance $\bv_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
% 	   \For{$t=1, ...,T$ }
% 	   \State Compute empirical estimator $\btheta_{t}=\bG_t^{-1}\bb_t$.
% 	   \State Construct two confidence sets, one for decision and one for the variance, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$, $C^{v}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\}$.
% 	   %\State $G_t=\lambda \boldsymbol{I} + \sum_{\tau < t}\bphi(i)\bphi(i)^{\top}$.
% 	   %$\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1, i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.
% 	   %\State Set UCB value $\bar{\mu}_{t,i}=\min \{\hat{\mu}_{t-1, i}+\rho_{t, i},1\}$.
% 	   \For{$i \in [m]$}
% 	   \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}} + 2\sqrt{\beta}\norm{\phi_{i}}_{\bG_t}$. // optimistic mean, double radius
% 	   \State $\ubar{\mu}_{t,i}=\inner{\bphi_t(i), \hat{\btheta}} - 2\sqrt{\beta}\norm{\phi_{i}}_{\bG_t}.$
% 	   \State Compute the optimistic variance by solving $\max_{\bnu \in C^{v}_t}{\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})}$ \begin{equation}
%     v_{t,i}= \begin{cases}
% (1-\bar{\mu}_{t,i})\bar{\mu}_{t,i}, &\text{if $\bar{\mu}_{t,i} \le \frac{1}{2}$}\\
% (1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}, &\text{if $\ubar{\mu}_{t,i} \ge \frac{1}{2}$}\\
% \frac{1}{4}, &\text{otherwise}.
% \end{cases}
% \end{equation} 
% \State Let $ \tilde{\bnu}_{t}(i), \tilde{\mu}_{t,i}$ are parameters that achieve $v_{t,i}$.
% 	   \EndFor
% 	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. 
% 	    \For{$ i \in S_t$ }
% 	   \State $\bG_t\pluseq v_{t,i}^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
% 	   \State $\bb_t\pluseq v_{t,i}^{-1}\bphi_{t}(i) X_{t,i}$.
% 	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
% 	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
% 	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
% 	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
% 	   % \label{line:trigger_upd}
% 	   \EndFor
% 	    	   \EndFor
% 		\end{algorithmic}
%           		\end{minipage}}
% \end{algorithm}

\begin{algorithm}[h]
	\caption{BC$^2$UCB-T: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Unknown Variance but with Monotonicity Assumption}\label{alg:BC^2UCB-T}
			\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, computation oracle ORACLE.
	   % \OUTPUT Budget allocation $\bk$.
	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0},$ optimistic variance $\bv_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
	   \For{$t=1, ...,T$ }
	   \State $\hat{\btheta_{t}}=\bG_{t-1}^{-1}\bb_{t-1}$. \Comment{Compute empirical estimator.}
	   %\State Construct two confidence sets, one for decision and one for the variance, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$, $C^{v}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\}$.
	   \For{$i \in [m]$}
	   \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + 2\sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}$.  \Comment{UCB value for arm $i$.}
	   \State $\bar{\mu}_{t,i}=\min \{\bar{\mu}_{t,i},1\}$.
	   \State $\ubar{\mu}_{t,i}=\inner{\bphi_t(i), \hat{\btheta}_t} - 2\sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}.$ \Comment{LCB value for arm $i$.}
	   \State $\ubar{\mu}_{t,i}=\max\{\ubar{\mu}_{t,i},0\}$.
	   %\State Compute the optimistic variance by solving $\max_{\bnu \in C^{v}_t}{\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})}$     
	   \State\begin{equation}\label{eq:var_upper}
 \bar{V}_{t,i}= \begin{cases}
(1-\bar{\mu}_{t,i})\bar{\mu}_{t,i}, &\text{if $\bar{\mu}_{t,i} \le \frac{1}{2}$}\\
(1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}, &\text{if $\ubar{\mu}_{t,i} \ge \frac{1}{2}$}\\
\frac{1}{4}, &\text{otherwise}.
\end{cases}
\end{equation} \Comment{Upper bound of the variance $V_i=(1-\mu_i)\mu_i$.}
% \State Let $ \tilde{\bnu}_{t}(i), \tilde{\mu}_{t,i}$ are parameters that achieve $v_{t,i}$.
	   \EndFor
	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. \Comment{Computational oracle using UCBs.}
	    \For{$ i \in \tau_t$ }\Comment{Update statistics.}\label{line:update_G}
	   \State $\bG_t=\bG_{t-1}+ \bar{V}_{t,i}^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
	   \State $\bb_t=\bb_{t-1}+ \bar{V}_{t,i}^{-1}\bphi_{t}(i) X_{t,i}$.\label{line:update_b}
	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
	   % \label{line:trigger_upd}
	   \EndFor
	    	   \EndFor
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}

As in \cref{alg:BC^2UCB-T}, for each arm $i$, we use $\bar{V}_{t,i}$ as an optimistic estimation of the variance. Indeed, $\bar{V}_{t,i}$ is the optimal value of the following problem, 
\begin{align}\label{eq:var_upper_explain}
\max_{\btheta \in C_t}{f_{t,i}(\btheta)=\inner{\bphi_t(i), \btheta}(1-\inner{\bphi_t(i), \btheta})}
\end{align}
where $C_t=\left\{\btheta: \norm{\btheta-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\right\}$ is the confidence ellipsoid for $\btheta^{*}$. To see why $\bar{V}_{t,i}$ takes the closed form as in \cref{eq:var_upper}, consider $f_{t,i}(x)=x(1-x)$ as a quadratic function of $x=\inner{\bphi_t(i), \btheta} \in [\ubar{\mu}_{t,i},\bar{\mu}_{t,i}]$. If $0.5 \in  [\ubar{\mu}_{t,i},\bar{\mu}_{t,i}]$, else if $\bar{\mu}_{t,i}\le 0.5$, max value is $\bar{\mu}_{t,i}(1-\bar{\mu}_{t,i})$, else if $\ubar{\mu}_{t,i} \ge 0.5$, max value is $(1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}$.

For notational convenience, we use $\tilde{\mu}_{t,i}=\argmax_{x} f_{t,i}(x)$ and $\bar{\bnu}_t(i)=\argmax_{\btheta}f_{t,i}(\theta)$ at round $t$ for arm $i$ as in \cref{eq:var_upper_explain}. Note that $\inner{\bphi_t(i),\bnu_t(i)}=\tilde{\mu}_{t,i}$. We also denote $\bar{\btheta}_{t}(i)$ be the vector that $\inner{\bphi_t(i),\bar{\btheta}_{t}(i)}=\bar{\mu}_{t,i}$.

\begin{align}
    &Reg(T)=\sum_{t=1}^T  r(S_t^*; \bmu)- r(S_t; \bmu)\\
    &\le \sum_{t=1}^T  r(S_t; \bar{\bmu}_{t})- r(S_t; \bmu) \\
    &\le \sum_{t=1}^T \abs{r(S_t; \bar{\bmu}_{t}) - r(S_t;\tilde{\bmu}_{t})} +\abs{ r(S_t; \tilde{\bmu}_t) - r(S_t; \bmu)}\\
    % & \mbox{$\tilde{\mu}_{t,i}, \tilde{\bnu}_{t}(i)$ are para. that achieve $v_{t,i}$}\\
    &\le\sum_{t=1}^T B_v \sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\bnu}_{t}(i)-\bar{\btheta}_{t(i)}, \bphi_t(i)}^2}{\bar{V}_{t,i}}} + B_v \sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\bnu}_{t}(i)-\btheta^*, \bphi_t(i)}^2}{\bar{V}_{t,i}}}& \mbox{(Apply \Cref{cond:VM} twice)}\\
    &\le\sum_{t=1}^T 2B_v \sqrt{\beta\sum_{i \in S_t}{\norm{ \bphi_t(i)/\sqrt{\bar{V}_{t,i}}}_{\bG_{t-1}^{-1}}^2}}  \\
    &\le  B_vd\sqrt{T}\log T 
\end{align}
\begin{remark}
The intuition of using variance is from the exploitation perspective: the smaller the variance, the more accurate the data point is, and thus more important for the agent to learn unknown $\btheta$. So we use the inverse of $\bar{V}_{t,i}$ in \cref{line:update_G} and \cref{line:update_b} to re-weight the observation.
\end{remark}

\subsection{Lower Bound for Contextual CMAB with Linear Reward}
Consider a $KT$ round linear bandit with $2^d$ feature vectors $\bx_t(i)\in\{-1,1\}^d$ and $\Theta=\{-1/\sqrt{T}, 1/\sqrt{T}\}$, each base arm's reward is $X_{t,i}==\inner{\bx_t(i), \btheta^*} + \eta_{t,i}$, where $\eta_{t,i}$ are independent. Then for any policy there exists a vector $\theta\in \Theta$ such that $R_T(A,\theta)\ge \Omega(d\sqrt{T})$ by Theorem 24.1 \cite{lattimore2020bandit}. For $KT$ rounds, if the algorithm can adaptively update each base arm observation, the regret is $\Omega(d\sqrt{KT})$.

\begin{remark}
Compared with the tabular case with independent base arms, where ESCB work~\cite{combes2015combinatorial} gives $\tilde{\Theta}(\sqrt{dT})$ regret, the lower bound of contextual CMAB has a $\sqrt{dK}$ gap. This gap comes from the fact that in the tabular case, base arms are independent and the feature vectors are orthogonal. In particular, the $\sqrt{d}$ term comes from the confidence coefficient $\beta$, where ESCB has order $\beta={O}(\sqrt{d+\log T})$, while LinUCB gives $\beta=\sqrt{d{\log T}}$ (though for fix-design actions, this can be relaxed in Eq. (20.3) to $\beta={O}(\sqrt{d+\log T})$~\cite{lattimore2020bandit}). The $\sqrt{K}$ term comes from that the arm feature vector in contextual CMAB could lie in the same direction (or exactly the same vector), and prevents the $\sqrt{K}$ improvement from ESCB.
\end{remark}

\subsection{Bandit Feedback is Sufficient to Match the Lower Bound}
Let $\Phi_t(S_t)=\sum_{i \in S_t}\bx_t(i)$, the reward $Y_t(S_t; \btheta)=\inner{\btheta, \Phi_t(S_t)} + \sum_{i \in S_t}\eta_t(i)$, which is a $\sqrt{K}$-subGaussian random variable. Following the linear bandit algorithm, we use pair oracle to select $\Phi_t(S_t)$ based on confidence ball $C_t$, the regret is $O(d\sqrt{KT})$~\cite{abbasi2011improved}.

\subsection{Contextual CMAB with Triggering Arms}
% Suppose we consider a simpler case, where $\bx_t$ is the context at round $t$, and $\E[\mu_a|\bx_t]=\inner{\bx_t, \theta_a}$. The triggered arms are $\tilde{S}_t$.

We start with the 1-norm TPM condition, and we have the following construction of the gram matrix and the $b$-value. For each round,

\begin{align}
    \bG_t&=\bG_{t-1}+\I\{i \in \tilde{A}_t\}\bphi_{t(i)}\bphi_{t(i)}^T.\\
    \bb_t&=\bb_{t-1}+\I\{i \in \tilde{A}_t\}\bphi_{t(i)}X_{t,i}.\\
    \hat{\btheta}_t&=\bG_{t-1}^{-1} \bb_{t-1}.
\end{align}

% \begin{align}
%     \tilde{G}_i(t)&=\tilde{G}_i(t-1)+p_i^{D,S_t}\bx_t^T \bx_t.\\
%     \tilde{b}_i(t)&=\tilde{b}_i(t-1)+p_i^{D,S_t}\bx_t r_t.\\
%     \hat{\btheta}_i(t)&=\tilde{G}_i(t)^{-1} \tilde{b}_i(t).
% \end{align}

Now for the regret, suppose $\alpha=\beta=1$, $\Delta_{S_t}=r(S_t^*;\btheta^*, \phi_t)-r(S_t;\btheta^*,\phi_t)$
\begin{align}
    Reg(T)&=  \E\left[\sum_{t=1}^T\Delta_{S_t}\right]\\
    &\le \E\left[\sum_{t=1}^T\sum_{i \in [m]}B_1p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)\right]\\
    &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1\E_{\tau_t}[\I\{i \in \tilde{A}_t\}](\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1\I\{i \in \tilde{A}_t\}(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in \tilde{A}_t}B_1(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\label{eq:trigger_prob_ieq}
\end{align}

For \cref{eq:trigger_prob_ieq}, it equals to the following,
\begin{align}
    &\E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}B_1(\bar{\mu}_{t,i}-\mu_i)\right]\\
    &\le \E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}B_1(\norm{\bar{\btheta}_t-\btheta^{*}}_{\bG_{t-1}}\cdot \norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}})\right]\\
    &\le B_1\sqrt{\beta}\E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}(\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}})\right]\\
    &\le B_1\sqrt{\beta}\E\left[\sqrt{KT \sum_{t=1}^T\sum_{i \in \tilde{A}_t}(\norm{\bphi_{t}(i)}^2_{\bG_{t-1}^{-1}})}\right]\\
    &\le B_1 \sqrt{d\log T} \sqrt{KT d\log(KT)}=B_1 d \sqrt{KT}\log(KT)
\end{align}
This gives the Contextual CMAB-T version under 1-norm TPM condition, which extends \citet{li2016contextual}.

Now if we use TPVM condition (and ignore $(1-\mu_i)\mu_i$ term for now), similarly, the regret is bounded by,
\begin{align}
     Reg(T)&=  \E\left[\sum_{t=1}^T\Delta_{S_t}\right]\\
    &\le \E\left[\sum_{t=1}^T B_v\sqrt{\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2}\right]\\
    &\le \E\left[ B_v\sqrt{T\sum_{t=1}^T\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2}\right]\\
    &\le B_v\sqrt{T} \sqrt{\E\left[\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2\right]}\\
    &\le B_v\sqrt{T} \sqrt{\E\left[\sum_{t \in T}\sum_{i \in \tilde{A}_t}(\bar{\mu}_{t,i}-\mu_i)^2\right]}\\
    &\le B_v\sqrt{\beta}\sqrt{T} \sqrt{\E\left[\sum_{t \in T}\sum_{i \in \tilde{A}_t}(\norm{\bphi_t(i)}_{\bG_{t-1}^{-1}}^2\right]}\\
    &\le d\sqrt{T}\log(KT).
\end{align}

This improves the Contextual CMAB-T with $\sqrt{K}$ factor under TPVM condition.


% For the regret, if we apply 1-norm bounded smoothness, we would have
% \begin{align}
%     Reg(T)&\le B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}( \bar{\mu}_{t,i}-\mu_i)\\
%     &\le  B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\inner{\bx_t,\bar{\theta}_i(t)-\theta_i}\\
%     &\le  B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\norm{\bx_t}_{G_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{G_i(t)}
% \end{align}
% If the last line is $B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\norm{\bx_t}_{\tilde{G}_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{\tilde{G}_i(t)}$, we can use $\tilde{\bx}_t=\sqrt{p_i^{D,S_t}}$ and prove the result using \begin{align}
%     &B_1\sum_{t}\sum_{i \in \tilde{S}_t}\norm{\tilde{\bx}_t}_{\tilde{G}_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{\tilde{G}_i(t)}\\
%     &\le B_1\sqrt{\beta} \sum_{i \in [m]}\sum_{t: i \in \tilde{S}_t} \sqrt{d N_i(T)\log T}\le B_1d\sqrt{\sum_{a}N_i(T)}\sqrt{\sum_{i} 1}\le B_1d\sqrt{mKT}.
% \end{align} However, we can only use $G_i(t)$, where $E[G_i(t)]=\tilde{G}_i(t)$? Or there is no difference?


\subsection{Technical Lemmas}

\begin{lemma}[Ellipsoidal potential lemma, \cite{abbasi2011improved}] Let $\bx_1,...,\bx_n$ be a sequence of vectors with $\norm{\bx_t}_2^2$, and let $G_t=I+\sum_{s=1}^{t-1}\bx_s \bx_s^T$. Then $\sum_{t=1}^n\min\{1,\norm{\bx_t}^2_{G_{t-1}^{-1}}\}\le 2 d \log (1+\frac{cn}{d}).$
\end{lemma}

\begin{lemma}[Theorem 3, \cite{lattimore2015linear}]
Let $\lambda>0, \delta=1/(TK), N=(4T^4d^2)^d, B\ge \max_{k}\norm{\btheta^*}_2^2,$ so that $\beta=(1+\sqrt{\alpha}+2\sqrt{\log\left(\frac{6TN}{\delta}\log\left(\frac{3TN}{\delta}\right)\right)})=O(\sqrt{d\log T})$. We have $\norm{\hat{\btheta}-\btheta_t}_{\bG_{t-1}}^2\le \beta$ for all $t\le T$ with probability at least $1-\delta=1$. 
\end{lemma}


\subsection{Next Steps}
\begin{enumerate}
    \item Plug in the details of the regret analysis (triggering \& variance parts).
    \item Check improved (?) analysis for 1-norm TPM condition without triggering groups.
    \item Check relation between the proof with pair oracles (Shuai's paper) and the proof with standard oracles (ours).
    \item Check upper and lower bound discussion (indicating whether or not our result is tight).
    \item Applications, e.g., cascading bandits, PMC, and rank-1 influence maximization.
\end{enumerate}
% \begin{itemize}
%     \item Confidence set and potential lemma for the unknown variance.
%     \item C$^2$MAB-T and triggering arms, one related RL paper using the peeling technique~\cite{he2021logarithmic}. Another work by \citet{demirel2021combinatorial} also considers TPM condition, where they use pseudo information gain to deal with the triggering arms.
%     \item Empirical Bernstein Inequality for self-normalized process, similar to the tabular case~\cite{audibert2009exploration}.
%     \item \sout{Lower bound for \citet{takemura2021near} is probably incorrect}.
%     \item Lower bound for contextual TPVM.
% \end{itemize}

==> content/x_new_analysis.tex <==
\clearpage
\section{A CMAB View of Episodic RL with Known Transition}
In this section, we first introduce the setup of episodic MDP and RL. Then we begin with a simple case of episodic RL, where transition kernels are known, to draw the connection between CMAB-T (i.e., CMAB-MT with $d=1$) and episodic RL. Based on this connection, we show that the general episodic RL with unknown transition is an instance of CMAB-MT. We also show how CMAB-MT framework can provide convenient plug-in algorithms/analysis for episodic RL, which matches the regret bound of the seminal work~\cite{jaksch2010near}.

\subsection{Episodic MDP and RL}\label{sec:setup_episodic_RL}
We consider the undiscounted finite horizon Markov Decision Process (MDP), i.e., episodic MDP, which can be described by a tuple $(\cS, \cA, H, \cP, \cR)$. $\cS$ is the finite state space with cardinality $S$. $\cA$ is the finite action space with cardinality $A$. $H$ is the horizon or the length of each episode. $\cP=(\bp(s,a,h))_{(s,a,h) \in \cS \times \cA \times [H]}$, where transition kernel $\bp(s,a,h)\in \Delta(\cS)$ and each element $p(s'|s,a,h)$ is the probability of transitioning to state $s'$ after taking action $a$ in state $s$ at horizon $h$.\footnote{We consider the general inhomogeneous setting where $\bp(s,a,h)$ at different horizons are different.} For the ease of exposition, reward distribution $\cR=(r(s,a,h))_{(s,a,h) \in \cS \times \cA \times [H]}$ are assumed to be Bernoulli random variables with mean $r(s,a,h)\in [0,1]$, indicating the instantaneous reward collected after taking action $a$ in state $s$ at horizon $h$. 

In episodic RL, the agent interacts with an unknown episodic MDP environment (where $\cP$ and/or $\cR$ are unknown) in a sequence of episodes $k \in [K]$ as follows: At the beginning of episode $k$, the agent starts from arbitrary initial state $s_{k,1}$ and determines a policy $\pi_k$, where $\pi_{t}(s,h) \in \cA$ maps any state and horizon $h$ to actions. Then at the $h=1,..., H$ step, the agent repeatedly selects an action $a_{t,h}=\pi_{t}(s,h)$,
receives a random reward $R_{k,h} \in [0,1]$ with mean $r(s_{t,h},a_{t,h},h)$, and randomly transits to next state $s_{t,h+1}$ with probability $p(s_{t,h+1}\mid s_{t,h}, a_{t,h}, h)$. The trajectory $(s_{t,h}, a_{t,h})_{h \in [H]}$ and the random reward $(R_{k,h})_{h \in [H]}$ are observed as feedback to improve future policies. 

Each policy $\pi$ identifies a value function for every state $s$ and horizon $h$ (i.e., the expected total reward starting from state $s$ at horizon $h$ until the end of the episode), defined as $V_{h}^{\pi}(s)=\E[\sum_{i=h}^H r(s_{i}, a_i, i)\mid s_h=s, \pi]$, where the expectation is taken over visited state-action pairs $(s_i, a_i)$ upon starting from state $s$ at horizon $h$. The optimal policy $\pi$ is indicated with $\pi*$ with its value function $V^{\pi^*}$. The objective of episodic RL is to minimize the regret, which is defined as $\text{Reg}(K)\overset{\text{def}}{=}\sum_{k \in [K]}\left(V_{1}^{\pi^*}(s_{k,1})-V_1^{\pi}(s_{k,1})\right)$.
\xutong{Bellman equation here}

\subsection{Episodic RL with Known Transition}

For an episodic RL with known transition described by $(\cS, \cA, H, \cP, \cR)$ as in \cref{sec:setup_episodic_RL},where the reward distribution $\cR$ is unknown, and needs to be learned by the agent, while the transition kernel $\cP$ is assumed to be known. 

\textbf{Problem Instance.} To show the connection between CMAB-MT and Episodic RL with known transition, we identify a CMAB-MT instance $([m], d, \Pi, \cD, \cD_{\text{trig}}, R)$ that fits this simple episodic RL. Specifically, there are $m=SAH$ base arms and each base arm $(s,a,h)$ corresponds to the instantaneous reward when state-action is $(s,a)$ at horizon $h$. Dimension $d=1$ since the instantaneous reward is a univariant random variable. The set of distributions $\cD$ are the episodic MDPs with the transition kernel being exactly $\cP$ and any possible reward distribution. $\Pi$ corresponds to the set of deterministic policies $\pi$ that maps any state and horizon $h$ to actions, i.e., $\pi: \cS \times [H] \rightarrow \cA$. The probabilistic triggering function $D_{\text{trig}}$ and the reward function $R$ will be specified later on.

\textbf{Learning Process.} For the learning process, the environment first generates a distribution $D \in \cD$, which is the episodic MDP with known transition kernel $\cP$ and unknown reward distribution $\cR$. In episode $k = 1, ..., K$, the environment $D$ generates Bernoulli random reward $\bX_{k}=(X_{k, s,a,h})_{(s,a,h) \in \cS\times \cA \times [H]}$ for each base arm $(s,a,h)$. After the agent executes policy $\pi_k$, a set of base arms $\tau_k=\{(s_{t,h}, a_{t,h}, h)\}_{h \in [H]}$ will be triggered, whose instantaneous reward $R_{k,h}=X_{k,s_{t,h}, a_{t,h},h}$ are then received and observed as feedback.

\textbf{Connection with CMAB-MT.} In this context, the reward function is $R(\pi_k, \bX_k, \tau_k)=\sum_{h \in [H]} R_{k,h}$, the triggering distribution $D_{\text{trig}}(\pi_k, \bX_k)$ is the distribution jointly determined by $\cP$ and $\pi$. 
Under episodic MDP $D$, the mean vector is $\bmu = (\mu_{s,a,h})_{(s,a,h)\in \cS \times \cA \times [H]} \in [0,1]^{SAH \times 1}$, where $\mu_{s,a,h}$ corresponds to the mean reward $r(s,a,h)$ for state-action $(s,a)$ at horizon $h$. And the expected combinatorial reward $r(\bmu; \pi)$ is exactly the value function $V_1^{\pi}(s_{1})=\E[R(\pi_k, \bX_k,\tau_k)]=\E[\sum_{h \in [H]}R_{k,h}]$.

Next, we validate the key quantity and conditions. For triggering probability $p_{s,a,h}^{D, \pi}$, it corresponds to the occupancy measure, i.e., $p_{s,a,h}^{D,\pi}(s,a,h)\overset{def}{=}\E[\I\{s_h=s, a_h=a\mid \pi, \cP\}]$, indicating the probability of visiting state-action pair $(s,a)$ at horizon $h$ when the underlying transition is $\cP$ and the policy is $\pi$. The batch size $K=H$ since $|\tau_k|=H$ by definition. For the monotonicity ( \cref{cond:mono}) and smoothness condition ( \cref{cond:general_smooth}), they are satisfied by the following lemma.

\begin{lemma}\label{thm:RL_known_smoothness}
    Episodic RL with known transition $(\cS, \cA, H, \cP, \cR)$ is a CMAB-MT instance, which satisfies monotonicity (\cref{cond:mono}) and 1-norm MTPM smoothness (\cref{cond:general_smooth}) with smoothness coefficient $B_1=1$ and distance function $w_i^{\tilde{\bmu},\bmu,\pi}=1$, i.e.,
    \begin{align}
    \abs{r(\pi;\tilde{\bmu})-r(\pi;\bmu)}\le \sum_{s,a,h}p_{s,a,h}^{\bmu, \pi} \cdot \abs{\tilde{r}(s,a,h)-r(s,a,h)}\end{align}
\end{lemma}

Since $X_i\in \{0,1\}$ are Bernoulli random variables, we use the empirical Bernstein inequality for each base arm, so the confidence region becomes $\cC_t=\{\tilde{\bmu}:|\tilde{\mu}_i-\hat{\mu}_{t-1,i}|\le \sqrt{\frac{3\hat{V}_{t-1,i}\log t}{T_{t-1,i}}}+\frac{2\log t}{T_{t-1,i}}\}$, where $\hat{V}_{t-1,i}$ is the empirical variance for arm $i$ before before (not including) $t$ rounds. Owing to the monotonicity condition, we identify the range oracle $\tilde{O}$ to be value iteration with $\cP$ and $\bar{\mu}_{t,i}=\hat{\bmu}_{t-1,i}+F_{t,i}\sqrt{\frac{1}{T_{t-1,i}}}+G_{t,i}\frac{1}{T_{t-1,i}}$, where $F_{t,i}=3\sqrt{\hat{V}_{t-1,i}\log t}, G_{t,i}=2\log t$.

For the analysis, we first use Bernstein inequality to show with high probability $F_{t,i}\sqrt{\frac{1}{T_{t-1,i}}}+G_{t,i}\frac{1}{T_{t-1,i}}\le \sqrt{12\Var[X_i]\log t}\sqrt{\frac{1}{T_{t-1,i}}}+28\log t\frac{1}{T_{t-1,i}}\}$ 

The following regret is achievable.XXX

\xutong{Algorithm is the value iteration with UCB rewards.}

\section{A CMAB View of Episodic RL with Unknown Transition}

In this section, we consider the setting of episodic RL $(\cS, \cA, H, \cP, \cR)$, where the transition kernel $\cP$ is unknown while the reward distribution $\cR$ is known.  

\textbf{Problem Instance.} From the CMAB-MT view, episodic MDP is a CMAB-MT instance $([m], d, \Pi, \cD, \cD_{\text{trig}}, R)$ as follows: there are $m=SAH$ base arms and each base arm $(s,a,h)$ corresponds to the unknown transition kernel $\bp(s,a,h) \in \Delta(\cS)$ when state-action is $(s,a)$ at horizon $h$. Dimension $d=S$ since the random transition is a multi-variant random variable that follows the categorical distribution with $S$ possible outcomes. The set of distributions $\cD$ are the episodic MDPs with any feasible transition kernels and the reward distribution being exactly $\cR$. $\Pi$ corresponds to the set of deterministic policies $\pi$ that maps any state and horizon $h$ to actions, i.e., $\pi: \cS \times [H] \rightarrow \cA$. The probabilistic triggering function $D_{\text{trig}}$ and the reward function $R$ will be specified later on.

\textbf{Learning Process.} For the learning process, the environment first generates a distribution $D=(\cP, \cR) \in \cD$, which is the episodic MDP with the unknown transition kernel $\cP$ and the known reward distribution $\cR$. In each episode $k = 1, ..., K$, the environment $D$ generates one-hot random transition vectors $\bdelta_{k,s,a,h}$ and Bernoulli random rewards $R_{k, s,a,h}$ for each base arm $(s,a,h) \in \cS\times \cA \times [H]$. Essentially, we can see that the outcome vector $\bX_k=(\bdelta_{k,s,a,h},R_{k,s,a,h})_{(s,a,h)\in \cS \times \cA \times [H]}$. After the agent executes policy $\pi_k$, a set of base arms $\tau_k=\{(s_{t,h}, a_{t,h}, h)\}_{h \in [H]}$ will be triggered, which determines the transition trajectories  ${(s_{t,h}, a_{t,h})_{h \in [H]}}$ and are observed as feedback.

\textbf{Connection with CMAB-MT.}
In episodic RL, the reward function is $R(\pi_k, \bX_k, \tau_k)=\sum_{h \in [H]} R_{k,h}$, the triggering distribution $D_{\text{trig}}(\pi_k, \bX_k)$ is the distribution jointly determined by $\cP$ and $\pi$. 
Under episodic MDP $D$, the mean vector is $\bmu = (\bp_{s,a,h})_{(s,a,h)\in \cS \times \cA \times [H]} \in [0,1]^{SAH \times S}$, where $\mu_{s,a,h}$ corresponds to the transition kernel $\bp(s,a,h)$ for state-action $(s,a)$ at horizon $h$. And the expected combinatorial reward $r(\bmu; \pi)$ is exactly the value function $V_1^{\pi}(s_{1})=\E[R(\pi_k, \bX_k,\tau_k)]=\E[\sum_{h \in [H]}R_{k,h}]$.

Next, we validate the key quantity and conditions. For triggering probability $p_{s,a,h}^{D, \pi}$, it corresponds to the occupancy measure, i.e., $p_{s,a,h}^{\pi,\cP}(s,a,h)\overset{def}{=}\E[\I\{s_h=s, a_h=a\mid \pi, \cP\}]$, indicating the probability of visiting state-action pair $(s,a)$ at horizon $h$. The batch size $K=H$ since $|\tau_k|=H$ by definition. For the monotonicity ( \cref{cond:mono}), though larger $\bmu$ corresponds to larger value function $V_1^{\pi}(s_1)$, there does not exist any two valid transition kernels $\bmu>\bmu'$. Therefore, monotonicity is meaningless. For the smoothness condition (\cref{cond:general_smooth}), it is satisfied by the following lemma.

% \begin{lemma}
%     Episodic RL with unknown transition $(\cS, \cA, H, \cP, \cR)$ is a CMAB-MT instance, which satisfies 1-norm MTPM smoothness (\cref{cond:general_smooth}) with smoothness coefficient $B_1=H$, distance function $\psi_{i}(\bmu, \bmu')=\norm{\bp_{s,a,h}-\bp'_{s,a,h}}_1$, i.e., $
%     \abs{V_1^{\bp,\pi}(s_1)-V_1^{\bp',\pi}(s_1)}\le H\cdot\sum_{s,a,h}p_{s,a,h}^{D, \pi} \cdot \left(\bp(s,a,h)-\bp'(s,a,h)\right)$
% \end{lemma}

\begin{lemma}
    Episodic RL with unknown transition $(\cS, \cA, H, \cP, \cR)$ is a CMAB-MT instance, which satisfies 1-norm MTPM smoothness (\cref{cond:general_smooth}) with smoothness coefficient $B_1=H$ and weight vector $\bw_i^{\tilde{\bmu},\bmu,\pi}=H\cdot\boldsymbol{1}$, i.e., $
    \abs{V_1^{\tilde{\bp},\pi}(s_1)-V_1^{\bp,\pi}(s_1)}\le H\cdot\sum_{s,a,h}p_{s,a,h}^{\tilde{\bp}, \pi} \cdot \norm{\tilde{\bp}(s,a,h)-\bp(s,a,h)}_1$.
\end{lemma}

Here $\bX_i\in \{0,1\}^d$ are multinoulli random variables, we use the concentration for multinoulli distributions, i.e., $\norm{\bp(s,a,h)-\hat{\bp}_{t-1}(s,a,h)}_1\le \sqrt{\frac{2S\log (2T/\delta)}{N_{t-1}(s,a,h)}}$ with probability at least $1-\delta$. So the confidence region becomes $\cC_t=\{\tilde{\bp}:\norm{\tilde{\bp}(s,a,h)-\hat{\bp}_{t-1}(s,a,h)}_1\le \sqrt{\frac{2S\log (2T/\delta)}{N_{t-1}(s,a,h)}},\tilde{\bp}(s,a,h)\in \Delta_{S} \text{, for all } s,a,h\}$. Based on the confidence region, the range oracle outputs $(\pi_t,\bp_t)=\argmax_{\pi\in \Pi, \tilde{\bp}\in \cC_t}V_1^{\tilde{\bp},\pi}(s_1)$, which can be solved by the extended value iteration~\cite{jaksch2010near} in $O(S^2AH)$ or linear program. See the appendix for details.

The regret is $O(H^2\sqrt{SAT})$ by \cref{thm:reg_CMAB-MT}.

\subsection{Achieving Minimax Optimal Regret by Incorporating RL Structures}\label{sec:va_c2mab}
In this section, we incorporate RL structures for improved 1-norm MTPM smoothness condition, confidence region $\cC_t$, and variance-aware analysis, which achieves minimax optimal regret for episodic RL.

\begin{lemma}
    Episodic RL with unknown transition $(\cS, \cA, H, \cP, \cR)$ is a CMAB-MT instance, which satisfies 1-norm MTPM smoothness (\cref{cond:general_smooth}) with weight vector $\bw_{i}^{\tilde{\bmu},\bmu,\pi}=\bV_{h+1}^{\tilde{\bmu},\pi}$,  i.e., $
    \abs{V_1^{\tilde{\bp},\pi}(s_1)-V_1^{\bp,\pi}(s_1)}\le \sum_{s,a,h}p_{s,a,h}^{\bmu, \pi} \cdot \abs{[\tilde{\bp}(s,a,h)-\bp(s,a,h)]^{\top} \bV_{h+1}^{\tilde{\bp},\pi}}$.
\end{lemma}

Using the RL structure, we use the following confidence region for action-transition pair $(\pi, \tilde{\bp})$ whose expected future value $\tilde{\bp}(s,a,h)^{\top}\bV^{\tilde{\bp},\pi}_{h+1}$ is bounded, i.e.,
\begin{align}
    &\abs{[\tilde{\bp}(s,a,h)-\hat{\bp}_t(s,a,h)]^{\top}V_{h+1}^{\tilde{\bp},\pi}}\le \phi_{t}(s,a,h)\\
 &\tilde{\bp}(s,a,h)\in \Delta_{S}.
\end{align}
% \begin{align}
%     &\abs{[\tilde{\bp}(s,a,h)-\hat{\bp}_t(s,a,h)]^{\top}V_{h+1}^{\tilde{\bp},\pi}}\le \phi_{t,s,a,h}\\
%     &V^{\pi}_{h}(s)=r(s,\pi_h(s),h)+\tilde{\bp}(s,\pi_h(s),h)^{\top}\bV^{\tilde{p},\pi}_{h+1}\\
%     &\bV_{H+1}^{\pi}=\boldsymbol{0}, \tilde{\bp}(s,a,h)\in \Delta_{S}.
% \end{align}
for all $s\in \cS, a\in h\in [H]$, where $\phi_{t}(s,a,h)$ is the confidence radius. Suppose $\phi_{t,s,a,h}$ is known, we can show that the range oracle over $\cC_t$, i.e., $(\pi^*_t,\tilde{\bp}^*_t)=\argmax_{\tilde{\bp}\in \cC_t}V_1^{\tilde{\bp},\pi}(s_1)$, is the value iteration with bonus $\phi_{t,s,a,h}$.





% \begin{lemma}
%     Episodic RL with unknown transition $(\cS, \cA, H, \cP, \cR)$ is a CMAB-MT instance, which satisfies 1-norm MTPM smoothness (\cref{cond:general_smooth}) with smoothness coefficient $B_1=1$, and let action-dependent distance function $\psi_{i}^{\pi}(\bmu, \bmu')=\abs{[\bp(s,a,h)-\bp'(s,a,h)]^{\top} V^{\pi,\bp'}_{h+1}}$ and distance function $\psi_i=\max_{\pi \in \Pi}\psi_i^{\pi}.$  i.e., $
%     \abs{V_1^{\bp,\pi}(s_1)-V_1^{\bp',\pi}(s_1)}\le \sum_{s,a,h}p_{s,a,h}^{D, \pi} \cdot \abs{[\bp(s,a,h)-\bp'(s,a,h)]^{\top} \bV_h^{\bmu',\pi}}$
% \end{lemma}

\begin{algorithm}[t]
	\caption{Optimistic Value Iteration Oracle in Episode $t$}\label{alg:v-opt}
		\resizebox{.93\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \STATE \textbf{Input:} Counter $N_{t-1}(s,a,h)$, empirical transition $\hat{\bp}_{t-1}(s,a,h)$ for all $s,a,h$.  
	   % \OUTPUT Budget allocation $\bk$.
	   \STATE \textbf{Initialize:} Constant $L=\logL$, value function $\bar{V}_{H+1}(s)=\ubar{V}_{H+1}(s)=0$.
    \FOR{ $h=H, H-1, ..., 1$}
    \STATE For all $(s,a)$, set confidence radius $\phi_{t}(s,a,h)=2\sqrt{\frac{\Var_{s'\sim \hat{\bp}(s,a,h)}\left(\bar{V}_{t,h+1}(s')\right)L}{N_{t-1}(s,a,h)}}+2\sqrt{\frac{\E_{s'\sim \hat{\bp}_{t-1}(s,a,h)}\left[\bar{V}_{t,h+1}(s')-\ubar{V}_{t,h+1}(s')\right]^2L}{N_{t-1}(s,a,h)}}+\frac{5HL}{N_{t-1}(s,a,h)}$.
    \STATE For all $(s,a)$, compute $Q_t(s,a,h)=r(s,a,h)+\min\left\{ \hat{\bp}_{t-1}(s,a,h)^{\top}\bar{\bV}_{t,h+1},\max_{s}\bar{V}_{t,h+1}(s)\right\}$.
    \STATE For all $s$, set $\pi_t(s,h)=\argmax_{a}Q_t(s,a,h)$.
    \STATE For all $s$, set $\bar{V}_{t,h}(s)=Q_t(s,\pi(s,h),h)$.
    \STATE For all $s$, set $\ubar{V}_{t,h}(s)=\max\{r(s,\pi(s,h),h)+\hat{\bp}_{t-1}(s,\pi(s,h),h)^{\top}\ubar{V}_{t,h+1}-\phi_t(s,a,h),\,\,0\}$.
    \ENDFOR
    \STATE \textbf{Return:} $\pi_t$.
		\end{algorithmic}   
				\end{minipage}}
\end{algorithm}

\begin{algorithm}[t]
	\caption{Extended Value Iteration Oracle in Episode $t$}\label{alg:ext_VI}
		\resizebox{.93\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \STATE \textbf{Input:} Counter $N_{t-1}(s,a,h)$, empirical transition $\hat{\bp}_{t-1}(s,a,h)$ for all $s,a,h$.  
	   % \OUTPUT Budget allocation $\bk$.
	   \STATE \textbf{Initialize:} $\phi'_t(s,a,h)=\frac{}{}$ Value function $\bar{V}_{H+1}(s)=0$ for all $s,a,h$.
    \FOR{Horizon $h=H, H-1, ..., 1$}
    \STATE For all $(s,a)$, set $\tilde{\bp}_t(s,a,h)=\argmax_{\tilde{}}$
    \STATE For all $(s,a)$, set $Q_t(s,a,h)=r(s,a,h)+\max_{\tilde{\bp}(s,a,h)\in \cC_t}\tilde{\bp}(s,a,h)^{\top}\bar{\bV}_{t+1}$.
    \STATE For all $s$, set $\pi(s,h)=\argmax_aQ_t(s,a,h)$ and $\bar{V}_h(s)=Q_t(s,\pi(s,h),h)$
    \ENDFOR
    \STATE \textbf{Return:} $\pi_t$.
		\end{algorithmic}   
				\end{minipage}}
\end{algorithm}


% \begin{algorithm}[t]
% 	\caption{Value-Optimistic Oracle}\label{alg:v-opt}
% 		\resizebox{.93\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
% 	\begin{algorithmic}[1]
% 	    \STATE \textbf{Input:} Constants $B_p,B_v, J, L$, variance function $g(\bp,\bV)=L\sqrt{\text{Var}_{\bp}(\bV)}$, confidence interval $\phi(\bp, \bV, s,a,h)=\frac{g(\bp,\bV)}{\sqrt{n_{k}(s,a,h)}}+\frac{J}{n_{k}(s,a,h)}$, failure probability $\delta$. 
% 	   % \OUTPUT Budget allocation $\bk$.
% 	   \STATE \textbf{Initialize:} Counter $n_k(s,a,h)=0, n_k(s,a,s',h)=0$, value function $\bar{V}_{H+1}(s)=0$.
%     \FOR{Episode $k=1,2, ...,$ }
%     \FOR{Horizon $h=H, H-1, ..., 1$}
%     \STATE For all $(s,a)$, compute empirical transition $\hat{\bp}(s,a,h)=\frac{n_k(s,a,\cdot, h)}{n_k(s,a,h)}$, confidence bound for next-state value $\phi_k^{\text{pv}}(s,a,h)=\phi(\hat{\bp}, \bar{\bV}_{k,h+1}, s,a,h)+\frac{B_v\norm{\bar{\bV}_{k,h+1}-\ubar{\bV}_{k,h+1}}_{2,\hat{\bp}}}{\sqrt{n_k(s,a,h)}}+\frac{B_p}{n_k(s,a,h)}$.
%     \STATE Compute upper next-state value $\bar{\bV}_{k, \text{next}}(s,a,h)=\hat{\bp}^{\top}(s,a,h)\bar{\bV}_{k,h+1} + \phi_k^{\text{pv}}(s,a,h)$ and lower next-state value $\ubar{\bV}_{k, \text{next}}(s,a,h)=\hat{\bp}^{\top}(s,a,h)\ubar{\bV}_{k,h+1} - \phi_k^{\text{pv}}(s,a,h)$.
%     \STATE $Q_k(a,h)=r(s,a,h)+\bar{\bV}_{k,\text{next}}(s,a,h)$.
%     \ENDFOR
%     \STATE Compute policy $\pi_k(s,h)=\argmax_{a\in \cA} Q_k(a,h)$.
%     \STATE Compute upper value function $\bar{\bV}_{k,h}(s)=Q_k(\pi_k(s,h), h)$.
%     \STATE Compute lower value function $\ubar{\bV}_{k,h}(s)=\min_{a\in\cA}\{r(s,a,h)+\ubar{\bV}_{k, \text{next}}(s,a,h)\}$.
%     \ENDFOR
%       \STATE Play action $\pi_k$, collect trajectory $(s_h,a_h,r(s_h,a_h,h))_{h\in[H]}$, and update statistics.
% 		\end{algorithmic}   
% 				\end{minipage}}
% \end{algorithm}
